PROPm Allocations of Indivisible Goods to Multiple Agents

We study the classic problem of fairly allocating a set of indivisible goods among a group of agents, and focus on the notion of approximate proportionality known as PROPm. Prior work showed that there exists an allocation that satisfies this notion of fairness for instances involving up to five agents, but fell short of proving that this is true in general. We extend this result to show that a PROPm allocation is guaranteed to exist for all instances, independent of the number of agents or goods. Our proof is constructive, providing an algorithm that computes such an allocation and, unlike prior work, the running time of this algorithm is polynomial in both the number of agents and the number of goods.

==> Algorithm.tex <==
Our algorithm begins by choosing some arbitrary agent $i\in N$ to serve as the ``divider'' (we henceforth use $i$ to refer to the divider agent and $N^{-i}=N\setminus\{i\}$ to refer to the set of all other agents). The divider agent partitions the items into $n$ bundles, and then the algorithm proceeds to evaluate the other agents' preferences over the other bundles in order to decide which one the divider should receive. Once the divider's bundle has been determined, the initial problem is reduced to smaller sub-problems that are solved recursively.

One of the appealing properties of our solution, is that the description of the algorithm is rather straightforward, and most of the complexity of our argument appears in proving the correctness of this algorithm, i.e., that it always returns a valid PROPm allocation (see Section~\ref{sec:correctness}).

\subsection*{Stage 1: the divider partitions the goods}
In order to partition the goods, the divider (agent $i$) first sorts them in non-decreasing order of value, from $i$'s perspective, and indexes them accordingly. Then, the first bundle $S_1$ corresponds to the longest prefix of goods in this ordering such that $v_i(S_1)\leq 1/n$. Observe that, by construction, $v_i(S_1) + v_i(g) > 1/n$ for all $g \in M\setminus S_1$.  Moreover, there is at least $(n-1)/n$ total value remaining for $i$ outside $S_1$.  We construct $S_{2}$ by taking the longest prefix of goods in $M \setminus S_1$ such that $i$ has value less than or equal to $1/(n-1) \cdot v_i(M \setminus S_1)$ for receiving all of them. Similarly, we let $S_k$ be the longest prefix of goods in $M \setminus (\cup_{j=1}^{k-1} S_j)$ such that the divider has value less than or equal to $1/k \cdot v_i(M \setminus (\cup_{j=1}^{k-1} S_j))$.
\vnote{Maybe add an example with actual numbers and, say, 2-3 agents? Not sure if this is worth it, though.}

\subsection*{Stage 2: decomposing into sub-problems}

Using the disjoint simple bundles $S_1, S_2, \dots, S_n$ defined by the divider's partition, we now decompose the problem into sub-problems, which we solve recursively. Specifically, we carefully choose one of these $n$ simple bundles, say $S_t$, and allocate it to the divider, and then we recursively allocate the items of bundles $S_1, \dots, S_{t-1}$ to some group $N_L$ of $t-1$ agents in $N^{-i}$, and the items of bundles $S_{t+1},\dots, S_n$ to some group $N_R$ of $n-t$ agents.

To choose which simple bundle to allocate to the divider agent, and how to decompose the agents in $N^{-i}$ into the two groups, $N_L$ and $N_R$, we repeatedly use a subroutine, \textsc{SeekPropDec} which, given a set of $k$ agents and a set of $k$ simple bundles, checks whether it is possible to decompose these sets into proportional sub-problems. If such a proportional decomposition is possible, the subroutine returns true, and otherwise returns false. Our algorithm (Algorithm \ref{alg:PROPm}) exhaustively searches through the $n$ possible assignments to the divider agent, and the partitions of the other agents into sets $N_L$ and $N_R$, and then uses the subroutine to check whether this choice could yield a proportional decomposition. If the answer is positive, then the decomposition is decided and the induced sub-problems are solved recursively, leading to the final allocation.

\vnote{Provide some discussion regarding how the subroutine works, or maybe defer that to the running time section.}


\begin{algorithm}%[H]
\DontPrintSemicolon
Let $S_1, S_2, \dots, S_n$ be the divider's simple bundles\;
$S_0 \leftarrow \emptyset$\;
\For{$t=1$ \KwTo $n$}
{
    \For{each $N_L\subseteq N^{-i}$ such that $|N_L|=t-1$}
    {
        $N_R \leftarrow N^{-i}\setminus N_L$\;
        L $\leftarrow$ \textsc{SeekPropDec}($(S_1,\dots, S_{t-1}), N_L$)\;
        \vnote{The next step could just check whether agents in $N_R$ prefer right collection}\;
        R $\leftarrow$ \textsc{SeekPropDec}($(S_{t+1},\dots, S_n), N_R$)\;
        \If{both $L$ and $R$ are true}
            {
                Allocate $S_t$ to agent $i$ (divider agent)\;
                Solve each sub-problem recursively\;
                Return the final allocation\;
            }
    }
}
 \caption{PROPm Algorithm}\label{alg:PROPm}
\end{algorithm}
\vnote{Check that the algorithmic environment is compatible with IJCAI and/or update it to look good}

\subsection*{Correctness and Running time}
As we discuss in Section~\ref{sec:running-time}, although the running time of this algorithm increases exponentially in the number of agents, its running time is polynomial in the number of items, leading to a polynomial running time for any fixed number of agents. This is in contrast to the algorithm proposed in \cite{PROPm}, whose running time was exponential in the number of items, even for a fixed number of agents.




==> correctness.tex <==
In order to verify the correctness of the algorithm, we first show that it always terminates and returns an allocation. As we verify in subsection~\ref{sec:correctSubroutine}, a single call to \textsc{UpdateDecomposition} subroutine returns an updated decomposition that has either increase in size by 1, or has reduced the value of $c$ by 1. Since the value of $c$ at the beginning of each iteration can never be more than $n-1$, this ensures that the while loop will always terminate within a finite number of iterations. If for some iteration $t\leq n-1$ the value of $c$ becomes 0, then the algorithm recurses on smaller problems and returns the induced allocation. If, on the other hand, $c$ does not drop to 0 for any $t\leq n-1$, then when $t=n$ we have an empty set $N_R$, necessarily leading to a value of 0 for $c$ in that iteration.

\subsection{Correctness of \textsc{UpdateDecomposition}}\label{sec:correctSubroutine}
We now formally prove that after every execution of the \textsc{UpdateDecomposition} subroutine, either the size of $D$ increases by 1, or the value of $c$ drops by 1. First, note that the set $R$ of vertices that are reachable from agent $k$ is bound to be non-empty. This is due to the fact that $v_k(S_1\cup\dots\cup S_t)/t> 1/n$, i.e., the agent's average bundle value is more than $1/n$ and, by pigeonhole principle, there must exist some sub-problem $(\bundleCollection, \agents')$ such that $v_k(\bundleCollection)/|\bundleCollection| \geq 1/n$. 

In the previous section we discussed how this subroutine re-arranges the agents across sub-problems along a path to vertex $w_\beta$ or to a vertex $i'$. In each of these cases it is easy to verify that the size of $D$ increases by 1 and the value of $c$ decreases by 1, respectively. But, we now also need to show that if neither one of these paths exists, the subroutine can find an alternative solution.

\begin{lemma}\label{lem:value_bound}
If $\bundleCollection'$ is the collection of all the simple bundles corresponding to sub-problems that are not reachable from $w_\beta$, excluding $S_t$, then for every agent $q$ from a sub-problem in $R$ we have $v_{q}(\bundleCollection')/|\bundleCollection'| < 1/n$. The same is true for the agent $k$ that corresponds to vertex $w_\alpha$, i.e., $v_k(\bundleCollection')/|\bundleCollection'| < 1/n$.
\end{lemma}
%\begin{lemma}
%Suppose that the {\metabundle}s in $D_j \cup \hat{D}$ consist of $t$ simple bundles.  Then all agents $k$ from vertices in $D$ have $v_{k}(D_j \cup \hat{D}) < t/n$.
%\end{lemma}
\begin{proof}
Assume that this is not the case, i.e., that either some agent $q$ corresponding to a sub-problem in $R$, or agent $k$, has an average bundle value at least $1/n$ for the simple bundles in $\bundleCollection'$. By pigeonhole principle, this implies that there must exist some sub-problem not reachable from $R$ such that this agent's average value for the bundles in that sub-problem is at least $1/n$. But, based on the definition of the sub-problem graph, this would imply the existence of an edge from that agent's vertex to this sub-problem's vertex, contradicting the fact that the latter is not reachable from the former.
%We proceed via contradiction.  Suppose that some agent $k'$ from a vertex in $D$ has $v_{k'}(D_j \cup \hat{D}) \geq t/n$.  We first note by our argument above that for all agents $k$ in {\metabundle}s corresponding to vertices in $D$ that $v_k(D_j) < 1/n$.  It must then be that $v_{k'}(\hat{D}) > (t-1)/n$.  Since this is a {\metaallocation} there are at most $t-1$ agents assigned to bundles in $\hat{D}$.  Moreover, no {\metabundle}s in $\hat{D}$ are {\unassigned} since this is a proportional {\incomplete} {\metaallocation} and $D_j$ is the {\unassigned} {\metabundle}.  However, we note that $\hat{D}$ has no incoming edges, so there must not be any agent who would retain {\propValue} at least $1/n$ if she were to replace an agent from one of the {\metabundle}s in $\hat{D}$.  In particular, this is true for agent $k'$.  So the value that $k'$ has for any {\metabundle} $\metaB$ in $\hat{D}$ is strictly less than $\frac{1}{n} \cdot |N'|$.  Since there are weakly fewer than $t-1$ agents assigned to {\metabundle}s in $\hat{D}$ we have that $v_{k'}(\hat{D}) \leq (t-1)/n$, a contradiction.
\end{proof}

%\begin{lemma}
%Suppose that the {\metabundle}s in $D_j \cup \hat{D}$ consist of $t$ simple bundles.  Then agent $i'$ has $v_{i'}(D_j \cup \hat{D}) < t/n$.
%\end{lemma}
%\begin{proof}
%The proof proceeds nearly identically as above.  It must be that $v_{i'}(D_j) < 1/n$ by definition.  Moreover, since $\hat{D} \cap D_1 = \emptyset$ we know that $i'$ would not have $\propValue$ at least $1/n$ if she were to replace some agent in any {\metabundle} corresponding to vertices in $\hat{D}$. Thus we know that the value $i'$ has for the items in any {\metabundle} $\metaB$ in $\hat{D}$ is strictly less than by $\frac{1}{n} \cdot |N'|$. Then, since $\hat{D}$ is comprised of $t-1$ simple bundles, it must be that $v_{i'}(\hat{D}) < (t-1)/n$.
%\end{proof}

Since agent $k$ and all agents $q$ from vertices in $R$ prefer the left collection at step $s$, we know that their overall value for the $s$ simple bundles in $S_1\cup \dots \cup S_s$ is greater than $t/n$. Lemma~\ref{lem:value_bound} implies that their total value for the simple bundles in $\bundleCollection'$ is less than $|\bundleCollection'|/n$. Therefore, these agents' value for the items corresponding to the sub-problems in $R$ is at least $(t-|\bundleCollection'|)/n$. 

Also, note that the overall number of agents in the sub-problems of $G$ (excluding $k$) is $t-1$, and the number of agents in the sub-problems not reachable from $R$ are $|\bundleCollection'|$, so the total number of agents in the sub-problems of $R$ is $t-|\bundleCollection'|-1$. Therefore, if we define a new sub-problem using the agents from $R$, combined with agent $k$ corresponding to vertex $w_\alpha$, and the simple bundles from $R$, combined with $S_t$, then this sub-problem will be proportional, because every agent's value for the simple bundles in it will be at least $(t-|\bundleCollection'|)/n$ and the number of agents in it is $t-|\bundleCollection'|$. 

\subsection{All agents are PROPm-satisfied}
To verify that the induced allocation is always PROPm, we first restate a useful observation from \cite{PROPm}. This observation provides us with a sufficient condition under which ``locally'' satisfying $\propXt$ in each sub-problem yields a ``globally'' $\propXt$ allocation. Given an allocation of a subset of items to a subset of agents, we say that this partial allocation is $\propXt$ if the agents involved would be $\propXt$-satisfied if no other agents or items were present.
%We are able to find allocations more readily because $\propXt$ is a more ``localized'' property than, say, EFx. 
%Provided that some subset of agents has enough total value for a given subset of items, we can recursively solve the problem on this smaller set of agents.  More concretely, at several points in the construction of $\propXt$ allocations we will use the following observation. 

\begin{observation}\label{obs:disjointAlloc}
Let $N_1, N_2$ be two disjoint sets of agents, let $M_1$ and $M_2 = M \setminus M_1$ be a partition of the items into two sets, and let $X$ be an allocation of the items in $M_1$ to agents in $N_1$ and items in $M_2$ to agents in $N_2$. Then, if some agent $i \in N_1$ is $\propXt$-satisfied with respect to the partial allocation of the items in $M_1$ to the agents in $N_1$, and $v_i(M_1) \geq \frac{|N_1|}{|N_1 + N_2|}$, then $i$ is $\propXt$-satisfied by $X$ regardless of how the items in $M_2$ are allocated to agents in $N_2$.  
\end{observation}
%\begin{proof}
%This follows from the definition of $\propXt$.  
%Fix some allocation $X$ of items in $M_1$ to agents in $N_1$ and items in $M_2$ to agents in $N_2$.  
%For all $i \in N_1$ we have $d_i(X) \geq \text{max}_{i' \in N_1\setminus\{i\}}\{\text{min}_{j \in X_{i'}}\{v_{ij}\}\}$.  Then, if $v_i(X_i) + \text{max}_{i' \in N_1\setminus\{i\}}\{\text{min}_{j \in X_{i'}}\{v_{ij}\}\} \geq \frac{v_i({M_1})}{|N_1|}$ (i.e., $i$ is $\propXt$ satisfied by $X$ with respect to the agents in $N_1$ and items in $M_1$) and $v_i(M_1) \geq \frac{|N_1|}{|N_1 + N_2|}$, it must be that $v_i(X_i) + d_i(X) \geq \frac{1}{n}$ so $i$ is also $\propXt$ satisfied by $X$ in the overall allocation of the items in $M$ to $N_1 \cup N_2$.
%\end{proof}


%\pnote{Do we need to include the following lemma?}
%We now observe that we may, without loss of generality, assume that  $v_{ij} \leq 1/n$ for every agent $i$ and item $j$.  

%\begin{lemma}
%If there exists some agent $i \in \agents$ and item $j \in \items$ such that $v_{ij} > 1/n$, we may allocate item $j$ to agent $i$ and reduce the problem to finding a $\propXt$ partial allocation of the items in $\items \setminus \{j\}$ to agents in $N\setminus\{i\}$.
%\end{lemma}
%\begin{proof}
% Let $X$ be an allocation which gives $j$ to agent $i$ and is a $\propXt$ allocation with respect to items in $\items \setminus \{j\}$ and agents in $N\setminus\{i\}$. Observe that agent $i$ is clearly $\propXt$ satisfied by $X$ (she is, in fact, proportionally satisfied).  If any other agent $i' \neq i$ also has value $v_{i'j} > 1/n$ for this item, then $d_{i'}(X)\geq 1/n$ (since $j$ is the only item in $X_i$). This implies that $i'$ is $\propXt$ satisfied since $v_{i'}(X_{i'}) + d_{i'}(X) \geq d_{i'}(X) \geq 1/n$.  Finally, all remaining agents $i'\neq i$ have $v_{i'j} \leq 1/n$ implying that $v_{i'}(\items \setminus \{j\}) \geq \frac{n-1}{n}$ and since $i'$ is $\propXt$ satisfied by $X$ with respect to the items in $\items \setminus \{j\}$ she must be $\propXt$ satisfied with respect to the entire allocation by Observation \ref{obs:disjointAlloc} substituting $N_1 = N \setminus \{i\}$ and $M_1 = M \setminus \{j\}$.
%\end{proof}

%As mentioned above, the $\spx$ sets for an agent play an integral role in our proof of the existence of $\propXt$ allocations. We start with an important property of the $\spxi{i}{n}{M}$ bundle for any agent. 

\vnote{Remove the following observation and move it to the place where it is used, not referring to CP sets.}
Their next observation provides some initial intuition regarding why $\spx$ sets play a central role in this paper.

%\vnote{Make sure that we are consistent with notation. E.g., I noticed the use of $M-S_n$ and $M\setminus S_n$ below. Also, are we should use ``$\propXt$ satisfied'' instead of ``satisfied by $\propXt$''}
\begin{observation}\label{obs:spxSatisfies}
If agent $i$ is allocated her $\spxi{i}{1}{\items}$ set, then $i$ is guaranteed to be $\propXt$-satisfied  regardless of how the other items are allocated. 
\end{observation}
%\begin{proof}
%Let $S$ be the $\spxi{i}{1}{\items}$ set of agent $i$ and consider an arbitrary allocation of $M \setminus S$ among the remaining $n-1$ agents.  By definition $v_i(S) + \min_{j \in M \setminus S}{v_{ij}} \geq 1/n$, so it must be that if $i$ is allocated $S$, she is $\propXt$ satisfied.
%\end{proof}


We now prove a result regarding the partition implied by the divider agent's preferences, which is an analogous to a theorem that is shown by \cite{PROPm} for a different, much more complicated, partition of the items.
\begin{theorem}\label{thm:recSpx}
Let $S_1, S_{2}, \dots, S_n$ be the simple bundles defined by the divider agent's partition. If this agent receives any bundle $S_{\ell}$ and no item from $S_1 \cup S_{2} \cup \cdots \cup S_{\ell - 1}$ is allocated to the same agent as an item from $S_{\ell + 1} \cup S_{\ell + 2} \cup \cdots \cup S_n$, then agent $i$ will be $\propXt$-satisfied.
%The agent will be PROPm satisfied if she receives any bundle $S_{\ell}$ for any allocation of the remaining items as long as the items in $S_n \cup S_{n-1} \cup \cdots \cup S_{\ell + 1}$ are in disjoint bundles from the items in $S_{\ell - 1} \cup S_{\ell - 2} \cup \cdots \cup S_1$. 
\end{theorem}
\begin{proof}
%The proof of this statement is not much harder than Observation~\ref{obs:spxSatisfies}.  
For all $k \in [n]$, we have $v_i(S_k) \leq \frac{1}{(n+1-k)}v_i(M \setminus (S_{1} \cup S_{2} \cup \dots \cup S_{k-1}))$ by definition of $S_k$.  Applying this upper bound on $v_i(S_k)$ for $k = 1$, because $v_i(M) = 1$ we have that $v_i(M\setminus S_1) \geq 1 - \frac{1}{n} = \frac{n-1}{n}$.  By  applying the upper bound on $v_i(S_k)$ for $k = 2$ and our lower bound on $v_i(M \setminus S_1)$ we get $v_i(M \setminus (S_1 \cup S_2)) \geq \frac{n-1}{n} - \frac{1}{n-1} \cdot \frac{n-1}{n} \geq \frac{n-2}{n}$.  Iteratively repeating this process, we obtain that for all $k \in [n]$ we know that $v_i(M \setminus (S_{1} \cup S_{2} \cup \dots \cup S_{k})) \geq \frac{n-k}{n}$.  Also by definition,  we have that $v_i(S_\ell) + \text{min}_{j \in M \setminus (S_{1} \cup S_{2} \cup \dots \cup S_{\ell})}\{v_{ij}\} \geq \frac{1}{(n+1-\ell)} \cdot v_i(M \setminus (S_{1} \cup S_{2} \cup \dots \cup S_{\ell-1})) \geq \frac{1}{n+1-\ell} \cdot \frac{n-(\ell-1)}{n} = \frac{1}{n}$.  But finally, as long as the items from $S_{1} \cup S_{2} \cup \dots \cup S_{\ell-1}$ are not included in any of the bundles containing the items in $M \setminus (S_{1} \cup S_{2} \cup \dots \cup S_{\ell})$ in the complete allocation $X$, we have that $d_i(X) \geq \text{min}_{j \in M \setminus (S_{1} \cup S_{2} \cup \dots \cup S_{\ell})}\{v_{ij}\}$ so $i$ is $\propXt$-satisfied when allocated set $S_{\ell}$.
\end{proof}

%Using these observations and constructions, we recursively construct a $\propXt$ solution for $n$ agents.  Our construction selects an arbitrary agent to be the ``divider'' who finds $n$ sets $\{S_i\}_{i \in [n]}$ as in Theorem \ref{thm:recSpx}.  We then aim to find an assignment of the remaining agents to these  such that we terminate with a $\propXt$ solution or a partition of these sets and the remaining agents such that we can recursively find a $\propXt$ solution on the subproblems. \pnote{Theorem 4 provides the crux for how we are always able to do this. It gives us the flexibility to always insert the divider agent into partitions where not enough agents have high value for the partition with the guarantee that the divider will be satisfied by PROPm}  By leveraging Observation \ref{obs:disjointAlloc}, these recursive solutions remain a $\propXt$ solution in the initial problem of $n$ agents. 


\subsection{Possibly useful definitions}
\vnote{Drop some of this paragraph's content.}
Proportional \metaallocation s will turn out to be crucial for our construction.  By Observation \ref{obs:disjointAlloc} for the agents in the {\metaallocation} we may recursively allocate goods to agents within the constituent {\metabundle}s and arrive at a solution that $\propXt$ satisfies all agents within the {\metaallocation}.  Possibly even more significant to our construction is the following definition.  We call a {\metaallocation} for a bundle collection $\bundleCollection$ and set of agents $\agents'$ \textbf{\incomplete} if the following three conditions are satisfied:
\begin{enumerate}
\item $|\bundleCollection| = |\agents'| + 1$
\item There is exactly one {\unassigned}  {\metabundle} containing exactly one simple bundle $A_j$
\item There is no {\metabundle} containing simple bundles which have indices below and above $j$ 
%\pnote{I don't think this condition is mentioned again later on. Maybe it makes sense to talk about this being a necessary condition for Theorem 4 to hold here.}
\vnote{Verify that we cannot just drop that this definition or this third bullet?}
\end{enumerate}

\vnote{Drop most of the following paragraph}
At the outset of our construction, we will ask an arbitrary agent to produce $n$ simple bundles of goods as in \ref{thm:recSpx}.  We will then consider a growing prefix of the ``left collection'' of these bundles.  At step $t$ of our analysis the left collection is the collection of bundles $(S_1, S_2, \dots S_t)$.  For the ordered collection of simple bundles $(S_1, S_2, \dots, S_n)$ we say that an agent \emph{prefers} the left collection (LC) at step $t$ if \[\sum_{i \in [t]}{v_j(S_i)} > \frac{t}{n}.\] 
\vnote{In some places we replaced this with weak inequality. Make sure that we use this consistently.}
For some set of agents $N'$ and step $t$ let $\lc{t}{N'}$ denote the subset of $N'$ who prefers the left collection at step $t$. \vnote{If we only use the size of this set, then we may as well define it as the number of agents that prefer the left collection rather than the set of them.}

\subsection{Proof of correctness}
Our proof proceeds inductively, that is to say, we show that for any number of agents $n$, we may arrive at a $\propXt$ allocation.  The base case is implied by the previous paper.  Our inductive hypothesis is straightforward, we assume that for any number $k < n$ of agents and any set of items we may find a $\propXt$ allocation of the goods to those agents.  By leveraging Observation \ref{obs:disjointAlloc}, we just then need to find some proportional {\metaallocation} to complete the proof since we may apply the inductive hypothesis on the \metabundle s therein.


For the first iteration, i.e., $t=1$, consider the value of $|\lc{1}{\agents^{-i}}|$.  If $|\lc{1}{\agents^{-i}}| = 0$, then we may give $S_1$ to $i$ (the divider) and by our inductive hypothesis, Observation \ref{obs:disjointAlloc}, and Theorem \ref{thm:recSpx} we may arrive at a $\propXt$ allocation by recursively finding a $\propXt$ solution among $n-1$ bidders on the set of items $\items \setminus S_1$.  If $|\lc{1}{\agents^{-i}}| > 0$ we may temporarily assign the left collection ($S_1$) to any agent in $\lc{1}{\agents^{-i}}$.  Let $N_1$ be the singleton set containing this agent.  The assignment of $S_1$ to the agent in $N_1$ is a proportional {\metaallocation}.  We then proceed to step $2$.


\subsection{Steps $2$ through $s$}
In step $2$, we consider the value of $|\lc{2}{\agents^{-i} \setminus N_1}|$.  If $|\lc{2}{\agents^{-i} \setminus N_1}| = 0$, then we may award $S_2$ to $i$ and recursively construct a $\propXt$ allocation using the proportional {\metaallocation} of $S_1$ to $N_1$ and recursively construct a $\propXt$ allocation of the right collection to the $n-1$ agents in $N^{-i} \setminus N_1$.  By our inductive hypothesis, Observation \ref{obs:disjointAlloc}, and Theorem~\ref{thm:recSpx} this will produce a $\propXt$ allocation.  

On the other hand, suppose that $|\lc{2}{\agents^{-i} \setminus N_1}| > 0$.  If there exists some set $N_2 \subset N^{-i}$ of size $2$ such that there is a proportional {\metaallocation} of the left collection at step $2$ and $N_2$, we proceed to step $3$.  If there does not exist such a set, we iterate through the subsets $N'_1 \subseteq N^{-i}$ of cardinality $1$ to find a proportional {\incomplete} {\metaallocation} for the left collection at step $2$ and $N'_1$ producing the lowest $|\lc{2}{\agents^{-i} \setminus N'_1}|$.  Note that, since we proceeded to step $2$, an {\incomplete} {\metaallocation} must exist. The proportional {\metaallocation} of the left collection from step $1$ to $N_1$ creates an {\incomplete} {\metaallocation} by treating $S_2$ as the {\unassigned} {\metabundle}.

\begin{lemma}\label{lem:step2score}
If there exists no set $N_2\subseteq N^{-i}$ of size 2 that yields a proportional decomposition with simple bundles $S_1$ and $S_2$, then $|\lc{2}{\agents^{-i} \setminus N'_1}| = 0$.
\end{lemma}
\begin{proof}
We proceed via contradiction. Suppose that the minimum $|\lc{2}{\agents^{-i} \setminus N'_1}|$ is attained for some set $N'_1$ but this value is greater than $0$.  There must then be some agent $i' \in \agents^{-i} \setminus N'_1$ that prefers the left collection at step $2$, i.e., $v_{i'}(S_1 \cup S_2) > 2/n$.  
%Without loss of generality, assume that the {\unassigned} {\metabundle} is $S_2$.  Then it must be that $v_{i'}(S_2) < 1/n$ since we were unable to find a proportional {\metaallocation} \pnote{I don't think it's clear how this fact is used in the proof}.  
Also note that the agent $k \in N'_1$ must have $v_{k}(S_1 \cup S_2) > 2/n$ since otherwise we could exchange agent $k$ with agent $i'$ in $N'_1$ to obtain a lower value of $|\lc{2}{\agents^{-i} \setminus N'_1}|$.  But then $v_{i'}(S_1 \cup S_2) > 2/n$ and $v_{k}(S_1 \cup S_2) > 2/n$ implies that the set $N_2=\{i', k\}$, combined with simple bundles $S_1$ and $S_2$ would yield a proportional sub-problem (and hence also a proportional decomposition), contradicting the assumption that such a decomposition does not exist.
%$k$ and $i'$ both prefer the left collection at step $2$, there must exist a proportional {\metaallocation} of the left collection at step $2$ and $N'_1 \cup \{i'\}$ contradicting that we did not find one when we searched for it.  Thus, we have that $|\lc{2}{\agents^{-i} \setminus N'_1}| = 0$.
\end{proof}

Since by Lemma \ref{lem:step2score}, we know that $|\lc{2}{\agents^{-i} \setminus N'_1}| = 0$, we may recursively allocate the assigned  {\metabundle}s in this {\metaallocation} to $N'_1$, assign $i$ the {\unassigned} {\metabundle} from this {\metaallocation}, and recursively allocate the right collection among the remaining (strictly fewer than $n$) bidders to arrive at a $\propXt$ allocation by our inductive hypothesis, Observation \ref{obs:disjointAlloc}, and Theorem \ref{thm:recSpx}.

We now consider step $s$ for any $2 < s \leq n-1$. \vnote{Why are we using $s$ here for denoting the step instead of $t$, used earlier, which also avoids the awkward notation $S_s$.} We proceed in much of the same way as before, examining the value of $|\lc{s}{\agents^{-i} \setminus N_{s-1}}|$.  If $|\lc{s}{\agents^{-i} \setminus N_{s-1}}| = 0$ then we can assign the divider $S_s$, recursively find an allocation to bidders in $N_{s-1}$ using our proportional {\metaallocation} of the left collection at step $s-1$ and $N_{s-1}$ by our inductive hypothesis, and recursively find a $\propXt$ allocation of the items from the right collection of bundles to the agents in $N^{-i} \setminus N_{s-1}$ by our inductive hypothesis.  By Observation \ref{obs:disjointAlloc} and Theorem \ref{thm:recSpx}, this yields a $\propXt$ allocation.  

If, on the other hand, $|\lc{s}{\agents^{-i} \setminus N_{s-1}}| \geq 1$ we attempt to find some set $N_s \subseteq \agents^{-i}$ with $|N_s| = s$ such that there exists some proportional {\metaallocation} of the left collection at step $s$ and $N_s$.  If it exists, we proceed to step $s+1$.  If such a set does not exist, we consider the family $\mathcal{F}$ of all subsets $I \subseteq N^{-i}$ of size $s-1$ such that there exists a proportional {\incomplete} {\metaallocation} of the left collection at step $s$ and $I$ and select the $I^* \in \mathcal{F}$ producing the minimum $|\lc{s}{\agents^{-i}\setminus I^*}|$.  Note that, since we proceeded to step $s$, an {\incomplete} {\metaallocation} must exist. The proportional {\metaallocation} of the left collection from step $s-1$ to $N_{s-1}$ creates an {\incomplete} {\metaallocation} by treating $S_s$ as the {\unassigned} {\metabundle}.  

\begin{lemma}\label{lem:concludeAllocation}
If $|\lc{s}{\agents^{-i}\setminus I^*}| = 0$, then we may recursively produce a $\propXt$ allocation for all agents.
\end{lemma}
\begin{proof}
We allow the agents in $I^*$ to split their corresponding {\metabundle}s to arrive at a $\propXt$ allocation for them by our inductive hypothesis, give $i$ (the divider) the {\unassigned} {\metabundle}, and recursively find a $\propXt$ allocation of the items in the right collection bundles to agents in $N^{-i} \setminus I^*$ using our inductive hypothesis.  Since $|\lc{s}{\agents^{-i}\setminus I^*}| = 0$, these agents must have value at least $(n-s)/n$ for the right collection of bundles and by Observation \ref{obs:disjointAlloc} and Theorem \ref{thm:recSpx} our recursively constructed allocation is a $\propXt$ allocation of all of the goods in $\items$ to all of the agents in $\agents$.
\end{proof}

With Lemma \ref{lem:concludeAllocation} in hand, we now aim to show that $|\lc{s}{\agents^{-i}\setminus I^*}|$ must indeed be equal to $0$. \vnote{The statement of the following lemma is informal (``arrive at this phase'')}

\begin{restatable}{lemma}{stepSscore}\label{lem:stepSscore}
If we arrive at this phase of the construction, $|\lc{s}{\agents^{-i} \setminus I^*}| = 0$.
\end{restatable}

As this lemma is more complicated we defer the proof of it to Subsection \ref{sub:stepSProof} of the document.

\subsection{Step $n$}

If we arrive at step $n$, we may immediately begin a recursive solution using our inductive hypothesis and conclude with a $\propXt$ allocation in hand.  To see this, observe that we proceeded to step $n$ because we were able to find a proportional {\metaallocation} of the left collection at step $n-1$ and $N_{n-1}$.  $N_{n-1}$ is a subset of $\agents^{-i}$ of size $n-1$, i.e., the non-dividing agents.  We may then recursively find a $\propXt$ allocation of the left collection at step $n-1$ to $\agents^{-i}$ by our inductive hypothesis and allocate $S_n$ to the dividing agent.  By Observation \ref{obs:disjointAlloc} and Theorem \ref{thm:recSpx} we then produce a $\propXt$ allocation of all of the goods in $\items$ to all of the agents in $\agents$.

Because at any path in the execution of our construction we arrive at a $\propXt$ allocation, we may conclude the proof yielding Theorem \ref{thm:mainThm}.

\begin{theorem} \label{thm:mainThm}
There exists a $\propXt$ allocation of any number of goods to any number of agents with additive valuations. 
\end{theorem}

\subsection{Proof of Lemma \ref{lem:stepSscore}}\label{sub:stepSProof}
We begin by restating the Lemma \ref{lem:stepSscore} for convenience. \vnote{The statement of the following lemma is informal (``arrive at this phase'')}
\stepSscore*
\begin{proof}
We proceed via contradiction.  Suppose that the $|\lc{s}{\agents^{-i} \setminus I^*}| \geq 1$.  Then there must exist an agent $i' \in \agents^{-i} \setminus I^*$ that prefers the left collection at step $s$.  In other words, $v_{i'}(S_1 \cup S_2 \cup \dots \cup S_s) > s/n$.  Without loss of generality, let $S_j$ be the simple bundle from the only {\unassigned} {\metabundle} in the {\incomplete} {\metaallocation}.  Since we could not produce a proportional {\metaallocation} it must be that $v_{i'}(S_j) < 1/n$.  Also, since $i'$ prefers the left collection, it must be that $i'$ would have {\propValue} weakly greater than $1/n$ for some {\metabundle} in the {\incomplete} {\metaallocation} if $i'$ were to replace one agent in the {\metabundle} \anote{I am afraid that this sentence may be not obvious. because her we mix two concepts here., ie. {\incomplete} {\metaallocation} + replace an agent}.


%We now construct a ``\metabundle'' graph $G = (V,E)$ as follows.  We let the vertices be the {\metabundle}s from the optimal (in the sense of having the lowest number of agents outside the allocation who prefer the left collection) {\incomplete} {\metaallocation} of the left collection.  We construct a subset of vertices $D_1$ beginning with all vertices for which agent $i'$ would have {\propValue} weakly greater than $1/n$ if she were to replace the agent in the corresponding {\metabundle}.  Note that $D_1$ must have at least one vertex in it by the reasoning above.  For each vertex $u \in D_1$ we create a directed edge $(u,v)$ to every vertex $v$ if there is at least one agent in the {\metabundle} corresponding to $u$ who would have {\propValue} at least $1/n$ if she were to replace another agent in the {\metabundle} corresponding to $v$ or if $v$ corresponds to the {\unassigned} {\metabundle} and she has {\propValue} at least $1/n$ for it.  In other words, the agent in the {\metabundle} corresponding to $u$ would be proportionally satisfied if she were added to the {\metabundle} corresponding to $v$ and some agent were removed from it (or the {\metabundle} is {\unassigned}).  We continue adding outgoing edges from any vertex with at least one incoming edge which satisfies the condition above (i.e., some agent in the {\metabundle} would have {\propValue} at least $1/n$ if she replaced another agent in some other {\metabundle}) until we cannot add any new edges.

Let $G$ be the sub-problem graph induced by the sub-problems of decomposition above, and add to it one more vertex, corresponding to agent $i'$, with outgoing edges to all the sub-problems $(\bundleCollection, \agents')$ of the decomposition for which $\frac{\sum_{A_j\in \bundleCollection}v_{i'}(A_j)}{|\agents'|}\geq \frac{1}{n}$. Also, let $D$ denote the set of sub-problems that are reachable from this added vertex. 

Note that the vertex corresponding to the {\unassigned} {\metabundle} corresponding to the simple bundle $S_j$ is not in $D$.  If it was, we could produce a proportional {\metaallocation} by propagating the replacements along the path beginning the newly added vertex, corresponding to agent $i'$, and ending at the vertex corresponding to the {\unassigned} {\metabundle}.  Along this path, each agent retains {\propValue} at least $1/n$ and we also give $i'$ {\propValue} at least $1/n$ which would yield a proportional {\metaallocation}, a contradiction.  By a similar argument, we can also demonstrate the following lemma.

\begin{lemma}\label{lem:preferLeft}
All agents from {\metabundle}s corresponding to vertices in $D$ prefer the left collection at step $s$.
\end{lemma}
\begin{proof}
We can show this by contradiction.  Suppose that some agent in a {\metabundle} corresponding to some vertex in $D$ does not prefer the left collection.  Then, we can propagate the path of replacements until we arrive at this vertex and remove the agent from the {\metaallocation} altogether.  But then we still have a proportional {\incomplete} {\metaallocation} (since the vertex corresponding to the {\unassigned} {\metabundle} is not in $D$) and this new {\incomplete} {\metaallocation} has strictly fewer agents outside it who prefer the left collection, contradicting the minimality of our original {\metaallocation}.
\end{proof}



%Let $D_j$ denote the vertex corresponding to the {\unassigned} {\metabundle} $S_j$ and $\hat{D}$ be the vertices in $V \setminus (D \cup D_j)$.  We may upper bound the value that any bidders in {\metabundle}s corresponding to vertices in $D$ have for {\metabundle}s in $\hat{D} \cup D_j$.  Slightly abusing notation, we let $v_{k}(V')$ denote the value an agent $k$ has for the bundles comprising the {\metabundle}s corresponding to a set of vertices $V'$.

\begin{lemma}\label{lem:value_bound}
If $\bundleCollection'$ is the collection of all the simple bundles corresponding to sub-problems that are not in $D$, excluding the bundle $S_j$, then for every agent $k$ from a sub-problem in $D$ we have $v_{k}(\bundleCollection')/|\bundleCollection'| < 1/n$. The same is true for agent $i'$, i.e., $v_{i'}(\bundleCollection')/|\bundleCollection'| < 1/n$.
\end{lemma}
%\begin{lemma}
%Suppose that the {\metabundle}s in $D_j \cup \hat{D}$ consist of $t$ simple bundles.  Then all agents $k$ from vertices in $D$ have $v_{k}(D_j \cup \hat{D}) < t/n$.
%\end{lemma}
\begin{proof}
Assume that this is not the case, i.e., that either some agent $k$ corresponding to a sub-problem in $D$, or agent $i'$, has an average item value at least $1/n$ for the simple bundles in $\bundleCollection'$. By pigeonhole principle, this implies that there must exist some sub-problem not reachable from $D$ such that this agent's average value for the items in that sub-problem is at least $1/n$. But, based on the definition of the sub-problem graph, this would imply the existence of an edge from that agent's vertex to this sub-problem's vertex, contradicting the fact that the latter is not reachable from the former.
%We proceed via contradiction.  Suppose that some agent $k'$ from a vertex in $D$ has $v_{k'}(D_j \cup \hat{D}) \geq t/n$.  We first note by our argument above that for all agents $k$ in {\metabundle}s corresponding to vertices in $D$ that $v_k(D_j) < 1/n$.  It must then be that $v_{k'}(\hat{D}) > (t-1)/n$.  Since this is a {\metaallocation} there are at most $t-1$ agents assigned to bundles in $\hat{D}$.  Moreover, no {\metabundle}s in $\hat{D}$ are {\unassigned} since this is a proportional {\incomplete} {\metaallocation} and $D_j$ is the {\unassigned} {\metabundle}.  However, we note that $\hat{D}$ has no incoming edges, so there must not be any agent who would retain {\propValue} at least $1/n$ if she were to replace an agent from one of the {\metabundle}s in $\hat{D}$.  In particular, this is true for agent $k'$.  So the value that $k'$ has for any {\metabundle} $\metaB$ in $\hat{D}$ is strictly less than $\frac{1}{n} \cdot |N'|$.  Since there are weakly fewer than $t-1$ agents assigned to {\metabundle}s in $\hat{D}$ we have that $v_{k'}(\hat{D}) \leq (t-1)/n$, a contradiction.
\end{proof}

%\begin{lemma}
%Suppose that the {\metabundle}s in $D_j \cup \hat{D}$ consist of $t$ simple bundles.  Then agent $i'$ has $v_{i'}(D_j \cup \hat{D}) < t/n$.
%\end{lemma}
%\begin{proof}
%The proof proceeds nearly identically as above.  It must be that $v_{i'}(D_j) < 1/n$ by definition.  Moreover, since $\hat{D} \cap D_1 = \emptyset$ we know that $i'$ would not have $\propValue$ at least $1/n$ if she were to replace some agent in any {\metabundle} corresponding to vertices in $\hat{D}$. Thus we know that the value $i'$ has for the items in any {\metabundle} $\metaB$ in $\hat{D}$ is strictly less than by $\frac{1}{n} \cdot |N'|$. Then, since $\hat{D}$ is comprised of $t-1$ simple bundles, it must be that $v_{i'}(\hat{D}) < (t-1)/n$.
%\end{proof}

Since agent $i'$ and all agents $k$ from vertices in $D$ prefer the left collection at step $s$, by Lemma~\ref{lem:preferLeft}, we know that their overall value for the $s$ simple bundles in $S_1\cup \dots \cup S_s$ is greater than $s/n$. Lemma~\ref{lem:value_bound} implies that their total value for the simple bundles in $\bundleCollection'$ is less than $|\bundleCollection'|/n$. Therefore, these agents' value for the items corresponding to the sub-problems in $D$ is at least $(s-|\bundleCollection'|)/n$. 

Also, note that the overall number of agents in the sub-problems of $G$ (excluding $i'$) is $s-1$, and the number of agents in the sub-problems not reachable from $D$ are $|\bundleCollection'|$, so the total number of agents in the sub-problems of $D$ is $s-|\bundleCollection'|-1$. Therefore, if we define a new sub-problem using the agents from $D$, combined with agent $i'$, and the simple bundles from $D$, combined with $S_j$, this sub-problem will be proportional, because every agent's value for the simple bundles in it will be at least $(s-|\bundleCollection'|)/n$ and the number of agents in it is $s-|\bundleCollection'|$. 
%$v_{i'}(D \cup D_j) > s/n$ and $v_{k}(D \cup D_j) > s/n$.  Moreover, since there are $s$ simple bundles in total in the left collection at step $s$, it must be that we can form a {\metabundle} from all simple bundles in $D_j \cup D$ and agents in $i' \cup D$ for which all of these agents have {\propValue} at least $1/n$.  
This contradicts that we could not find a proportional {\metaallocation} of the left collection at step $s$ consisting of $s$ agents and completes our proof.
\end{proof}
